The Liar's Walk: Detecting Deception with Gait and Gesture

We present a data-driven deep neural algorithm for detecting deceptive walking behavior using nonverbal cues like gaits and gestures. We conducted an elaborate user study, where we recorded many participants performing tasks involving deceptive walking. We extract the participants' walking gaits as series of 3D poses. We annotate various gestures performed by participants during their tasks. Based on the gait and gesture data, we train an LSTM-based deep neural network to obtain deep features. Finally, we use a combination of psychology-based gait, gesture, and deep features to detect deceptive walking with an accuracy of 88.41%. This is an improvement of 10.6% over handcrafted gait and gesture features and an improvement of 4.7% and 9.2% over classifiers based on the state-of-the-art emotion and action classification algorithms, respectively. Additionally, we present a novel dataset, DeceptiveWalk, that contains gaits and gestures with their associated deception labels. To the best of our knowledge, ours is the first algorithm to detect deceptive behavior using non-verbal cues of gait and gesture.

==> ECCV2020 Tanmay Deception/1_introduction.tex <==
\section{Introduction}
\begin{figure}[t]
      \centering
      \includegraphics[width=\columnwidth]{images/cover}
      \caption{\textbf{Detecting Deception}: We present a new data-driven algorithm for detecting deceptive walking using nonverbal cues of gaits and gestures. We take an individual's walking video as an input, compute psychology-based gait features, gesture features, and deep features learned from a neural network, and combine them to detect deceptive walking. In the examples shown above, smaller hand movements (a) and the velocity of hands and feet joints (d) provide deception cues.}
      \vspace{-15pt}
      \label{fig:cover}
\end{figure}

% \begin{figure}
% \centering
% \includegraphics[height=6.5cm]{eijkel2}
% \caption{One kernel at $x_s$ ({\it dotted kernel}) or two kernels at
% $x_i$ and $x_j$ ({\it left and right}) lead to the same summed estimate
% at $x_s$. This shows a figure consisting of different types of
% lines. Elements of the figure described in the caption should be set in
% italics,
% in parentheses, as shown in this sample caption. The last
% sentence of a figure caption should generally end without a full stop}
% \label{fig:example}
% \end{figure}

% FIRST PARAGRAPH: APPLICATIONS WHERE DETECTING DECEPTIVE BEHAVIOR IS NECESSARY
In recent years, AI and vision communities have focused a lot on learning human behaviors, and human-centric video analysis has rapidly developed~\cite{wang2015video,wei2017deep,xu2016heterogeneous,mcduff2017large}. While conventional video content analysis pays attention to the analysis of the video content, human-centric video analysis focuses on the humans in the videos and attempts to obtain information about their behaviors, describe their dispositions, and predict their intentions. This includes recognition of emotions~\cite{kuo2018compact,lee2019context,marinoiu20183d}, personalities~\cite{wei2017deep,zhang2016deep}, and actions~\cite{wu2017recent,yao2019review}, as well as anomaly detection~\cite{nguyen2019anomaly,morais2019learning,sultani2018real}, etc. While these problems are being widely studied, a related problem, detecting deception, has not been the focus of much research.

Masip et al.~\cite{MasipDefiningDeception} define deception as ``the deliberate attempt, whether successful or not, to conceal, fabricate, and/or manipulate in any other way, factual and/or emotional information, by verbal and/or nonverbal means, in order to create or maintain in another or others a belief that the communicator himself or herself considers false''. Motives for deceptive behaviors can vary from inconsequential to those constituting a serious security threat. Many applications related to computer vision, human-computer interfaces, security, and computational social sciences need to be able to automatically detect such behaviors in public areas (airports, train stations, shopping malls), simulated environments, and social media~\cite{tsikerdekis2014online}. In this paper, we address the problem of automatically detecting deceptive behavior learned from gaits and gestures from walking videos.

% MOVE SOME OF THE REFERENCES AND TEXT BELOW TO SECTION 2 AND SIGNIFICANTLY CUT DOWN SECTION. ITS VERY LONG. ALMOST HITS PAGE 3 :) IT SHOULND'T BE MORE THAN 1.5 PAGES INCLUDING ABSTRACT, TITLE AND COVER IMAGE. ALSO CVPR IS 8+REFS, WE CAN DO SOME HACKS TO SHRINK SIZE/SPACE

Deception detection is a challenging task because deception is a subtle human behavioral trait, and deceivers attempt to conceal their actual cues and expressions. However, there is considerable research on verbal (explicit) and nonverbal (implicit) cues of deception~\cite{EkmanNonverbalLeakage}. Implicit cues such as facial and body expressions~\cite{EkmanNonverbalLeakage}, eye contact~\cite{Zuckerman1981}, and hand movements~\cite{JensenIdentification} can provide indicators of deception. Facial expressions have been widely studied as cues for automatic recognition of deception~\cite{ding2019face,michael2010motion,meservy2005deception,perez2015verbal,perez2015deception,hu2018deep,wu2018deception}. However, deceivers try to alter or control what they think is getting the most attention from others~\cite{EkmanTellingLies1985}. Compared to facial expressions, body movements such as gaits are more implicit and are less likely to be controlled. This makes gait an excellent avenue for observing deceptive behaviors. The psychological literature on deception also shows that multiple factors need to be considered when deciphering nonverbal information~\cite{Buller1996}.

% With the recent rapid development of human-centric AI, human-centric video analysis [48, 49, 54, 30, 32, 61, 27] has also begun to draw much attention from the computer vision community. Other than the conventional video content analysis that focuses on generic semantic concept analysis of video content, human-centric video analysis aims to extract, describe, and organize a wealth of information regarding the main objects of interest in most videos: humans. This topic covers a wide range of research problems such as deception detection [36, 37], emotion recognition in videos [54, 18], personality computing [49, 56], and action recognition [6, 26, 28, 35, 40, 47, 59]. For example, it is often important to recognize the deceptive behaviors [36, 37], emotions [54, 18], or personality traits [49, 56] of the subject of a video in real-world scenarios.

% When humans interact with each other, they form perceptions of the each other's emotions, moods, intentions, and personalities. These perceptions are useful for performing cooperative and competitive tasks. For human-computer interaction, automated approaches that detect emotions, moods, and personalities of individuals are being developed that can make these interactions more fluent and efficient~\cite{dagar2016automatic,stratou2015automatic,kaur2017automatic}. Instances of implicit behaviors such as gaits have been leveraged in a diverse range of HCI applications, including gaming~\cite{detection_hci_1}, coaching company executives~\cite{detection_hci_4}, developing smart domestic appliances~\cite{detection_hci_3}, etc. However, these applications assume that humans are being fair and not trying to deceive the computer, which is not always the case. 



%expediting the process of making parole decisions, police investigations, courtroom trials~\cite{courtroom} etc., can benefit immensely from unobtrusive and efficient detection of deception.



% Our work, on the other hand, enables the computer to detect deception using unobtrusive methods. This has the potential to be applied to a wide range of HCI applications DID PRIOR BEHAVIOR PAPERS IN CHI USE THESE SURVEILLANCE OR SECURITY AS HCI APPLICATIONS, such as detection of suspicious behaviors in public areas such as airports, train stations, shopping malls, expediting the process of making parole decisions, police investigations, etc. DO HUMANS RELY ON GAITS AND GESTURES IN THESE APPLICATIONS?


% The ability to detect deception would mean that we could detect potential criminals, make better parole decisions, 

% know when we're being lied to, and decrease the likelihood that liars get away with their deceitfulness. 

% If we could know when someone was lying, then we could know who to trust. We are faced with the decision of who to trust everyday. This research could help take the guess work out of the process. The applications could extend beyond petty crime. Parole decisions, standardized test-takers, concert security, and other situations that require us to decide whether someone might act deceitfully could benefit from our algorithm. THIS LOOKS GOOD. CAN WE ALSO ADD APPLICATIONS THAT AREN'T RELATED TO CRIME? I AM ALSO THINKING OF SOME AND WILL ADD THEM. -OK I WILL THINK ABOUT IT 

% isjudgments in most of these cases may lead to confusion, misunderstandings, and inefficiencies in the tasks. However, in some situations, these misjudgments can be literally a matter of life and death (for example, a jury deciding whether someone is lying or not). 


% A part of human nature is the give and take of everyday interactions. Humans feel a certain sense of obligation to return favors that are given to them, a natural aspect of reciprocity and cooperation. This means that we are making judgments everyday in order to decide who to invest in, and what exchanges will reap the most benefits ~\cite{GouldnerReciprocity}. This relates to deception because people that are deceitful would be less likely to participate in this exchange. By interacting with these people and contributing to the exchange, you would be giving resources to aid survival of the other person without gaining the same benefit. This is not optimal for survival. 


% SECOND PARAGRAPH: PSYCHOLOGICAL DEFINITION OF DECEPTION AND HOW HUMANS DETECT IT (VERBAL, NONVERBAL CUES, ETC?)

% HERE IS AN ARTICLE FOR DECEPTION FOR SOCIAL MEDIA (CITE): https://cacm.acm.org/magazines/2014/9/177936-online-deception-in-social-media/abstract (THOUGH IT IS ONLINE)

% According to Ekman, different areas of the body have different sending capacities that provide information based on the difference in the movement, visibility, and speed of transmission. Hands are able to express nearly as much info as the face ~\cite{EkmanNonverbalLeakage}.


% THIRD AND FORTH PARAGRAPH: WHY GAITS AND GESTURES ARE THE MOST IMPORTANT CUES AND WE FOCUS ON THEM



% On the other hand, prior work has shown that people have less conscious control over their eye movements, and  therefore, eye movements have been tracked to detect personalities and behaviors of individuals efficiently~\cite{detection_hci_2}. 

%combine body movements such as gait with gestures, and attempt to distinguish deceptive walks from natural walks.

% We also know from emotion research that assessing movements of the body is a more reliable way of reading the important information, such as affect ~\cite{Aviezer}. Alternatively to facial expressions, body movements are more implicit and may be less likely to be controlled.

% Hands are able to express nearly as much info as the face
\textbf{Main Results:} We present an data-driven approach for detecting deceptive walking of individuals based on their gaits and gestures as extracted from their walking videos (Figure~\ref{fig:cover}). Our approach is based on the assumption that humans are less likely to alter or control their gaits and gestures than facial expressions~\cite{EkmanTellingLies1985}, which arguably makes such cues better indicators of deception. 

% Our approach is based on gaits and gestures because these body expressions can communicate as much information about a person's behavior as facial expressions~\cite{Aviezer}. Additionally, humans are less likely to alter or control their gaits and gestures than they are their facial expressions~\cite{EkmanTellingLies1985}, which arguably makes such cues more authentic indicators of deception.

Given a video of an individual walking, we extract his/her gait as a series of 3D poses using state-of-the-art human pose estimation~\cite{dabral2018learning}.  We also annotate various gestures performed during the video. Using this data, we compute psychology-based gait features, gesture features, and deep features learned using an LSTM-based neural network. These gait, gesture, and deep features are collectively referred to as the \textit{deceptive features}. Then, we feed the deceptive features into fully connected layers of the neural network to classify normal and deceptive behaviors. We train this neural network classifier (\textit{Deception Classifier}) to learn the deep features as well as classify the data into behavior labels on a novel dataset (\textit{DeceptiveWalk}). Our Deception Classifier can achieve an accuracy of \accuracy~when classifying deceptive walking, which is an improvement of $4.7\%$ and $9.2\%$ over classifiers based on the state-of-the-art emotion~\cite{bhattacharya2019step} and action~\cite{shi2019skeleton} classification algorithms, respectively.

Additionally, we present our deception dataset, \textit{DeceptiveWalk}, which contains $2224$ annotated gaits and gestures collected from $162$ individuals performing deceptive and natural walking. The videos in this dataset provide interesting observations about participants' behavior in deceptive and natural conditions. Deceivers put their hands in their pockets and look around more than the participants in the natural condition. Our observations also corroborate previous findings that deceivers display the opposite of the expected behavior or display a controlled movement~\cite{EkmanNonverbalLeakage,DePauloCues,Navarro2003}. 

% We collected this dataset using a data collection user study, where participants performed either natural or deceptive walks. In each condition, the participant performed a task where they picked up an object from a designated location and exchanged it with a confederate. The deceptive walk is induced by the experimenter during the briefing, the type of object, and the appearance of the confederate. We collected videos of the participants walking and extracted their gaits and gestures. 

Some of the novel components of our work include:\\
\noindent 1. A novel deception feature formulation of gaits and gestures obtained from walking videos based on psychological characterization and deep features learned from an LSTM-based neural network.

\noindent 2. A novel deception detection algorithm that detects deceptive walking with an accuracy of \accuracy.

\noindent 3. A new public domain dataset, \textit{DeceptiveWalk}, containing annotated gaits and gestures with deceptive and natural walks.

The rest of the paper is organized as follows. In Section 2, we give a brief background on deception and discuss previous methods of detecting deceptive walking automatically. In Section 3, we give an overview of our approach and present the details of our user study. We also present our novel \textit{DeceptiveWalk} dataset in Section 3. We present the novel deceptive features in Section 4 and provide details of our  method for detecting deception from walking videos. We highlight the results generated using our method in Section 5.

==> ECCV2020 Tanmay Deception/2_related.tex <==
\section{Related Work}
In this section, we give a brief background of research on deception and discuss previous methods for detecting deceptive behaviors automatically.

\subsection{Deception}
Research on deception shows that people behave differently when they are being deceitful, and different clues can be used to detect deception~\cite{EkmanNonverbalLeakage}. Darwin first suggested that certain movements are ``expressive'' and escape the controls of the will~\cite{Darwin}. Additionally, when people know that they are being watched, they alter their behavior in something known as ``The Hawthorne Effect''~\cite{LevittHawthorneEffect}. To avoid detection, deceivers try to alter or control what they think others are paying the most attention to~\cite{EkmanTellingLies1985}. Different areas of the body have different communicating abilities that provide information based on differences in movement, visibility, and speed of transmission~\cite{EkmanNonverbalLeakage}. Therefore, using channels to which people pay less attention and that are harder to control are good indicators of deception. 

Body expressions present an alternative channel for perception and communication, as shown in emotion research~\cite{Aviezer}. Body movements are more implicit and may be less likely to be controlled compared to facial expressions, as evidenced by prior work, suggesting that clues such as less eye contact~\cite{Zuckerman1981}, downward gazing (through the affective experiences of guilt/sadness)~\cite{BaumeisterGuilt,EkmanTellingLies1985}, and general hand movements~\cite{JensenIdentification} are good indicators of deception. Though there is a large amount of research on non-verbal cues of deception, there is no single conclusive universal cue~\cite{vrij2019reading}. To address this issue, we present a novel data-driven approach that computes features based on gaits and gestures, along with deep learning.


%  Implicit cues such as facial and body expressions~\cite{EkmanNonverbalLeakage}, eye contact~\cite{Zuckerman1981}, and hand movements~\cite{JensenIdentification} can provide such non-controllable indicators of deception.

%  However, when people know that they are being watched, they alter their behavior in something known as ``The Hawthorne Effect''~\cite{LevittHawthorneEffect}. Deceivers try to alter or control what they think is getting the most attention from others~\cite{EkmanTellingLies1985}. In addition, some research suggests that facial expressions can be unpredictable and not align with what is expected~\cite{KrautSmiling}.

% Body expressions present an alternative channel for perception and communication, as shown in emotion research~\cite{Aviezer}. Compared to facial expressions, body movements such as gaits are more implicit and are less likely to be controlled. This makes gait an excellent avenue for observation of deceptive behaviors. The psychological literature on deception also shows that multiple factors need to be considered when deciphering nonverbal information~\cite{Buller1996}. Therefore, in this work, our goal is to exploit these features based on gaits and gestures.

\subsection{Automatic Detection of Deception}
Many approaches have been developed to detect deception automatically using verbal or text-based cues. Text-based approaches have been developed to detect deception in online communication~\cite{zhou2008following}, news~\cite{conroy2015automatic}, court cases~\cite{fornaciari2013automatic}, etc. A large number of approaches that detect deception using non-verbal cues have focused on facial expressions and head and hand gestures~\cite{perez2015verbal,perez2015deception,ding2019face,hu2018deep}. Some approaches use only facial expressions to detect deception~\cite{avola2019automatic,hasan2019facial}, while other approaches use only hand and head gestures~\cite{michael2010motion,meservy2005deception}. In situations where the subject is sitting and talking, Van der Zee et al.~\cite{van2019freeze} used full-body features captured using motion capture suits to detect deception. However, such an approach is impractical for most applications. Other cues that have been used for detecting deception include eye movements~\cite{zuo2019your}, fMRI~\cite{cui2013detection}, thermal input~\cite{buddharaju2005automatic,abouelenien2014deception}, and weight distribution~\cite{atlas2005detection}. Recent research has also introduced multimodal approaches that use multiple modalities such as videos, speech, text, and physiological signals to detect deception~\cite{gupta2019bag,rill2019high,wu2018deception,krishnamurthy2018deep,karimi2018toward,abouelenien2017gender,abouelenien2016detecting}. However, most of these approaches have focused on humans that have been sitting or standing; deception detection from walking is relatively unexplored. This is an important problem for many applications such as security in public areas (e.g., airports, concerts, etc.) and surveillance. Therefore, in this paper, we present an approach that detects deception from walking using gait and gesture features.

% DECEPTION:
% CVPR
% Face-Focused Cross-Stream Network for Deception Detection in Videos
% Bag-Of-Lies: A Multimodal Dataset for Deception Detection
% High-Level Features for Multimodal Deception Detection in Videos

% ECCV
% Motion Profiles for Deception Detection Using Visual Cues
% Deep Multi-Task Learning to Recognise Subtle Facial Expressions of Mental States

% AAAI
% Deception Detection in Videos

% IJCAI 
% Deception Stefan Sarkadi

% ARXIV
% a deep learning approach for multimodal deception detection

% Others
% Beyond the Truth Machine: Emerging Technologies for Lie Detection
% Toward End-to-End Deception Detection in Videos
% Automatic Deception Detection in RGB videos using Facial Action Units
% Airport artificial intelligence can detect deception: or am i lying?
% Automatic Long-Term Deception Detection in Group Interaction Videos
% To freeze or not to freeze: A culture-sensitive motion capture approach to detecting deceit
% Interpretable Multimodal Deception Detection in Videos
% Facial Expression Based Imagination Index and a Transfer Learning Approach to Detect Deception
% Your Eyes Say You're Lying: An Eye Movement Pattern Analysis for Face Familiarity and Deceptive Cognition
% Detection of deception based on fmri activation patterns underlying the production of a deceptive response and receiving feedback about the success of the deception after a mock murder crime.
% Deception Detection using Real-life Trial Data.
% A multimodal dataset for deception detection
% Gender-based multimodal deception detection
% Detecting deceptive behavior via integration of discriminative features from multiple modalities.

\subsection{Non-verbal Cues of Gaits and Gestures}
Research has shown that body expressions, including gaits and gestures, are critical for the expression and perception of others' emotions, moods, and intentions~\cite{kleinsmith2013affective}. Gaits have been shown to be useful in conveying and recognizing identity~\cite{wan2019survey}, gender~\cite{yu2009study}, emotions~\cite{kleinsmith2013affective}, moods~\cite{michalak2009embodiment}, and personalities~\cite{atkinson2007evidence,roether2009critical}. Gestures have also been widely observed to convey emotions~\cite{labarre1947cultural,noroozi2018survey}, intentions~\cite{mount2008intentions}, moods~\cite{de2006towards}, personality~\cite{ball1999relating}, and deception~\cite{michael2010motion,meservy2005deception,ding2019face,hu2018deep}. For gait recognition, many deep learning approaches have been proposed~\cite{zhang2019gait,zhang2019learning,wang2019ev}, and LSTM-based approaches have been used to model gait features~\cite{zhang2019gait}. Body expressions have also been used for anomaly detection in videos with multiple humans~\cite{morais2019learning}. Many deep learning approaches have been proposed to recognize and generate actions from 2D~\cite{khodabandeh2018diy,yang2018pose} and 3D skeleton data~\cite{shi2019skeleton,pavllo2018quaternet,habibie2017recurrent}. Graph convolution networks such as STEP~\cite{bhattacharya2019step} and ST-GCN~\cite{yan2018spatial} for emotion and action recognition from skeleton data respectively have also been proposed. Inspired by these approaches that showcase the communicative capability of gaits and gestures, we use these non-verbal cues to detect deceptive walks.


% CVPR Papers related to gait
% Joint Intensity and Spatial Metric Learning for Robust Gait Recognition
% Gait Recognition under Speed Transition
% Two-Point Gait: Decoupling Gait from Body Shape



% When humans interact with each other, there is a give and take of clues and 

% When people interact with each other, they make judgments in order to decide who to trust and in return be trusted. 

% A part of human nature is the give and take of everyday interactions. Humans feel a certain sense of obligation to return favors that are given to them, a natural aspect of reciprocity and cooperation. This means that we are making judgments everyday in order to decide who to invest in, and what exchanges will reap the most benefits ~\cite{GouldnerReciprocity}. This relates to deception because people that are deceitful would be less likely to participate in this exchange. By interacting with these people and contributing to the exchange, you would be giving resources to aid survival of the other person without gaining the same benefit. This is not optimal for survival. 

==> ECCV2020 Tanmay Deception/4_classification.tex <==
\section{Automatic Deception Detection}
From the user study, we obtain a dataset of 3D pose data for each video. Using this pose data, we extract gait and gesture features. We also compute deep features using a deep LSTM-based neural network. We use these novel deception features as input to a classification algorithm. In this section, we first describe these deception features and their computation. We then describe the classification algorithm.

\subsection{Gait Features}
\begin{table}[t]
\caption{\textbf{Posture Features}: In each frame, we compute the following features that represent the human posture.}
\centering
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{Type} & \multicolumn{1}{c|}{Description} \\ \hline
Volume & Bounding box \\ \cline{1-2}
\multirow{5}{*}{Angle At}
                                & Neck by shoulders \\ \cline{2-2}
                                & Right shoulder by neck and left shoulder \\ \cline{2-2}
                                & Left shoulder by neck and right shoulder\\ \cline{2-2}
                                & Neck by vertical and back  \\ \cline{2-2}
                                & Neck by head and back  \\ \cline{1-2}
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Distance \\ Between\end{tabular}}                                                           & Right hand and the root joint \\ \cline{2-2}
                                & Left hand and the root joint \\ \cline{2-2}
                                & Right foot and the root joint \\ \cline{2-2}
                                & Left foot and the root joint \\ \cline{2-2}
                                & Consecutive foot strikes (stride length) \\ \cline{1-2}
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Area of \\ Triangle\end{tabular}}                                                           & Between hands and neck \\ \cline{2-2}
                                & Between feet and the root joint \\ \hline
\end{tabular}
\vspace{-15pt}
\label{tab:posturefeatures}
\end{table}
% \end{wraptable}

In previous work~\cite{randhavane2019identifying}, researchers have used a combination of posture and movement features to represent a gait. This is based on the finding that both posture and movement features are used to predict an individual's affective state~\cite{kleinsmith2013affective}. These features relate to the joint angles, distances between the joints, joint velocities, and space occupied by various parts of the body and have been used to classify gaits according to emotions and affective states ~\cite{crenn2016body,kleinsmith2013affective,randhavane2019identifying}. Since deceptive behavior impacts the emotional and cognitive state of an individual~\cite{Slepian,EkmanNonverbalLeakage}, features that are indicators of affective state may also be related to deception. Therefore, we use a similar set of gait features for the classification of deceptive walks, as described below. Combining the posture and the movement features, we obtain $29$ dimensional gait features.

% KYRA, CAN YOU PLEASE FIND REFERENCES FOR RELATING THESE GAIT FEATURES TO DECEPTION?).
% Slepian et al. suggests in a study about the physical burden of secrecy that people bearing secrets are impacted behaviorally and cognitively. They report that walking distances seem farther, hills steeper, and they even overthrow an object at a target, perceiving the distance to the target as being greater than it really is ~\cite{Slepian}. This demonstrates a strong link between a distressing emotional burden like having a secret and the perceptions of the surrounding physical world. Along this line of research, we could expect that walking patterns/gait also be affected by carrying the burden of a lie. 


% We represent the extracted affective features of a gait $\textbf{G}$ as a vector $F \in \mathbb{R}^{29}$. 
% For feature extraction, we use a single stride from each gait corresponding to consecutive foot strikes of the same foot. We used a single cycle in our experiments because in some of the datasets (CMU, ICT, EWalk) only a single walk cycle was available. When multiple walk cycles are available, they can be used to increase accuracy.

\subsubsection{Posture Features}
In each frame, we compute the features relating to the distances between joints, angles between joints, and the space occupied by various parts of the body. These features correspond to the body posture in that frame. We use the 3D joint positions computed using the human pose extraction algorithm (Section~\ref{sec:poseExtraction}) to compute these posture features as described below:
\begin{itemize}[noitemsep,topsep=0pt]
    \item Volume: We use the volume of the bounding box around a human as the feature that represents the compactness of the human's posture.
    \item Area: In addition to volume, we also use the areas of triangles between the hands and the neck and between the feet and the root joint to model body compactness.
    \item Distance: We use the distances between the feet, the hands, and the root joint as features. These features model body expansion and also capture the magnitude of the hand and food movement.
    \item Angle: We use the angles extended by different joints at the neck to capture the head tilt and rotation. These features also capture whether the posture is slouched or erect using the angle extended by the shoulders at the neck.
    \item Stride Length: Stride length has been used to represent gait features in literature; therefore, we also include stride length as a posture feature. We compute the stride length by computing the maximum distance between the feet across the gait.
\end{itemize}
We summarize these posture features in Table~\ref{tab:posturefeatures}. There are $13$ posture features in total.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/neural_net.png}
    \caption{\textbf{Our Classification Network}: Each of the 3D pose sequences corresponding to various walking styles is fed as input to the LSTM module consisting of $3$ LSTM units, each of depth $2$. The output of the LSTM module (the deep feature pertaining to the 3D pose sequence) is concatenated with the corresponding gait feature and the gesture feature, denoted by the $\mathbf{\bigoplus}$ symbol. The concatenated features are then fed into the fully connected module, which consists of two fully connected layers. The output of the fully connected module is passed through another fully connected layer equipped with the softmax activation function to generate the predicted class labels.}
    \vspace{-15pt}
    \label{fig:neural_net}
\end{figure}

\subsubsection{Movement Features}
% \begin{table}[t]
% \caption{\textbf{Movement Features}: We compute features that represent the movement of the important joints of the body. These joints are decided according to studies in psychology and previous literature~\protect \cite{karg2010recognition,crenn2016body}.}
% \centering
% \begin{tabular}{|l|l|c|}
% \hline
% \multicolumn{1}{|c|}{Type}                                                         & \multicolumn{1}{c|}{Description} \\ \hline
% \multirow{5}{*}{Speed}                                                             & Right hand \\ \cline{2-2}
%                                                                                   & Left hand  \\ \cline{2-2}
%                                                                                   & Head \\ \cline{2-2}
%                                                                                   & Right foot \\ \cline{2-2}
%                                                                                   & Left foot  \\ \cline{1-2}
% \multirow{5}{*}{Acceleration Magnitude} & Right hand  \\ \cline{2-2}
%                                                                                   & Left hand \\ \cline{2-2}
%                                                                                   & Head \\ \cline{2-2}
%                                                                                   & Right foot  \\ \cline{2-2}
%                                                                                   & Left foot \\ \cline{1-2}
% \multirow{5}{*}{Movement Jerk}        & Right hand \\ \cline{2-2}
%                                                                                   & Left hand  \\ \cline{2-2}
%                                                                                   & Head  \\ \cline{2-2}
%                                                                                   & Right foot  \\ \cline{2-2}
%                                                                                   & Left foot  \\ \cline{1-2}
% Time                                                                               & One gait cycle   \\ \hline
% \end{tabular}
% \vspace{-15pt}
% \label{tab:movementfeatures}
% \end{table}

In addition to the human posture in each frame, movement of the joints across time is also an important feature of gaits~\cite{kleinsmith2013affective}. We model this by computing the magnitude of the speed, acceleration, and movement jerk of the hands, head, and foot joints.  For each joint, we compute these features using the first, second, and third finite derivatives of its 3D position computed using the human pose extraction algorithm. We also include the gait cycle time as a feature. We compute this by the time between two consecutive foot strikes of the same foot. There are $16$ movement features in total. We aggregate both posture and movement features over the gait to form the $29$ dimensional gait feature vector.
% We summarize the movement features in Table~\ref{tab:movementfeatures}. 


% Psychologists have shown that motion is an important characteristic for the perception of different emotions. High arousal emotions are more associated with rapid and increased movements than low arousal emotions. Since faster gaits are perceived as happy or angry whereas slower gaits are considered sad~\cite{karg2010recognition}, we also include the time taken for one walk cycle ($gt\in \mathbb{R}$) as a movement feature. 


% \subsubsection{Affective Features}
% We combine posture and movement features and define affective features $F$ as: $F = F_{m} \cup  F_{p}$.


\subsection{Gesture Features}
We use the set of gestures described in Section~\ref{sec:gestures} and formulate the gesture features as a $7$ dimensional vector corresponding to the set \{Hands In Pockets, Looking Around, Touching Face, Touching Shirt/Jackets, Touching Hair, Hands Folded, Looking at Phone\} $\in \mathbb{R}^7$. For each gesture $j$ in the set, we set the value of $G_i^j = 1$ if the gesture is present in the walking video and $G_i^j = 0$  if it is absent. For \textit{hands in pockets}, we use $G_i^j = 1$ if one hand is in the pocket, $G_i^j = 2$ if two hands are in the pocket, and $G_i^j = 0$  if no hands are in the pockets. 

\subsection{Deep Features}
Given a sequence of 3D pose data for a fixed number of time frames as input, the task of the classification algorithm is to assign the input one of two class labels --- natural or deceptive. To achieve this, we develop a deep neural network consisting of \textit{long short-term memory} (LSTM)~\cite{lstm} layers. LSTM units consist of feedback connections and gate functions that help them retain useful patterns from input data sequences. Since the inputs in our case are walking motions, which are periodic in time, we reason that LSTM units can learn to efficiently encode the different walking patterns in our data, which, in turn, helps the network segregate the data into the respective classes. We call the feature vectors learned from the LSTM layers, \textit{deep features}, $f_d \in \mathbb{R}^{32}$.

\subsection{Classification Algorithm and Network Architecture}
Our overall neural network is shown in Figure~\ref{fig:neural_net}. We first normalize the input sequences of 3D poses so that each individual value lies within the range of $0$ and $1$. We feed the normalized sequences of 3D poses into an LSTM module, which consists of $3$ LSTM units of sizes $128$, $64$, and $32$, respectively, and each of depth $2$. We concatenate the $32$ dimensional deep features (output from the LSTM module) with the $29$ dimensional gait and the $7$ dimensional gesture features and feed the $68$ dimensional combined deceptive feature vectors into a convolution and pooling module. This module consists of $2$ convolution layers. The first convolution layer has a depth of $48$ and a kernel size of $3$. It is followed by a maxpool layer with a window size of $3$. The second convolution layer has depth $16$ and a kernel size of $3$. The output of the second convolution layer is flattened and passed into the fully connected module, which consists of $2$ fully connected (FC) layers of sizes $32$ and $8$, respectively. All the FC layers are equipped with the ELU activation function. The output feature vectors from the fully connected module are passed through a $2$ dimensional fully connected layer with the softmax activation function to generate the output class probabilities. We assign the predicted class label as the one with a higher probability.

==> ECCV2020 Tanmay Deception/5_results.tex <==
% \begin{table}[t]
% \caption{\textbf{Classification}: We compared our method with state-of-the-art methods for gait-based action recognition as well as perceived emotion recognition. Both these classes of methods use similar gait datasets as inputs but learn to predict different labels.}
% \centering
% \label{tab:classification}
% \begin{tabular}{cccc}
% \toprule
% ST-GCN~\cite{yan2018spatial} & DGNN~\cite{shi2019skeleton} & STEP~\cite{bhattacharya2019step} & Ours \\
% \midrule
% $77.82\%$ & $79.19\%$ & $83.68\%$ & \accuracybold \\
% \bottomrule
% \end{tabular}
% \vspace{-5pt}
% \end{table}

\section{Results}
We first describe the implementation details of our classification network, followed by a detailed summary of the experimental results.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{\textbf{Accuracy and Ablation Study}: We compared our method with state-of-the-art methods for gait-based action recognition as well as perceived emotion recognition. Both these classes of methods use similar gait datasets as inputs but learn to predict different labels. Additionally, we evaluated the usefulness of the different features for classifying a walk as natural or deceptive. We observed that all three components of the deceptive features (gait features, gesture features, and deep features) contribute towards the accurate prediction of deceptive behavior.}
\label{tab:accuracy}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{ST-GCN~\cite{yan2018spatial}} & \multirow{2}{*}{DGNN~\cite{shi2019skeleton}} & \multirow{2}{*}{STEP~\cite{bhattacharya2019step}} & \multicolumn{5}{c|}{Ours}                                \\ \cline{4-8} 
                        &                       &                       & Gestures & Gait    & Gestures + Gait & Deep    & All     \\ \hline
77.82\%                 & 79.19\%               & 83.68\%               & 61.59\%  & 72.56\% & 77.74\%         & 82.67\% & \accuracybold \\ \hline
\end{tabular}
\end{table}

% \begin{table}[t]
% \caption{\textbf{Ablation Study}: We evaluated the usefulness of the different features and different classification algorithms for classifying a walk as natural or deceptive. We observed that all three components of the deceptive features (gait features, gesture features, and deep features) contribute towards the accurate prediction of deceptive behavior.}
% \centering
% \label{tab:ablation}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{rccccc}
% \toprule
% & \multicolumn{5}{c}{Features} \\
% \cline{2-6}
% & Gestures & Gait & Gestures and Gait \Tstrut & Deep & All Combined \\
% \midrule
% Random Forest \Tstrut \Bstrut & $60.6\%$ & $70.0\%$ & $74.0\%$ & $79.3\%$ & $84.6\%$ \\
% LSTM+FC \Tstrut \Bstrut & $61.59\%$ & $72.56\%$ & $77.74\%$ & $82.67\%$ & \accuracybold \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-15pt}
% \end{table}

\subsection{Implementation Details}
We randomly selected $80\%$ of the dataset for training the network, $10\%$ for cross-validation and kept the remaining $10\%$ for testing. Inputs were fed to the network with a batch size of $8$. We used the standard cross-entropy loss to train the network. The loss was optimized by running the Adam optimizer~\cite{adam} for $n = 500$ epochs with a momentum of $0.9$ and a weight decay of $10^{-4}$. The initial learning rate was $0.001$, which was reduced to half its present value after $250$ $\left(\frac{n}{2}\right)$, $375$ $\left(\frac{3n}{4}\right)$, and $437$ $\left(\frac{7n}{8}\right)$ epochs.

\subsection{Experiments}
We evaluate the performance of our LSTM-based network as well as the usefulness of the deep features through exhaustive experiments. All the experimental results are summarized in Table~\ref{tab:accuracy}.

% Since ours is the first algorithm that detects deception from walking gaits, we compare the performance of our algorithm with a random forest classification method. First, we feed all the features and feature combinations to an off-the-shelf random forest classifier with $100$ decision trees, each of max depth $2$. Each tree performs binary classification on sub-samples of the dataset, and the final estimate is calculated as a weighted average of the prediction of the individual trees. Random forest classifiers do not naturally capture the temporal patterns of the walking styles in the 3D pose sequences. Hence it leads to a lower accuracy compared to using an LSTM-based network. Moreover, since each tree in the Random Forest is a weak classifier and the final estimate is obtained by averaging, the performance is observed to be poorer than the LSTM-based network even when only the gait and gesture features are used for classification. Overall, we find a consistent $3\%$ improvement in accuracy across the board when using the LSTM-based network over the Random Forest classifier.

We compare the performance of using the LSTM-based network with the various input features individually. Gesture features by themselves provide the lowest classification accuracy because they only coarsely summarize the subject's activities and not their walking patterns. Gait features, on the other hand, contain only this information and are seen to be more helpful in distinguishing between the class labels. Gestures and gait features collectively perform better than their individual performances. However, these features still lose some of the useful temporal patterns in the original 3D pose sequences. Using LSTMs to learn the temporal patterns directly from the 3D pose sequences, we observe an improvement of $\sim 5\%$ over using the combined gait and the gesture features. Finally, combining the deep features learned from the LSTM module with the gait and gesture features leads to an overall classification accuracy of \accuracy.

Since ours is the first algorithm that detects deception from walking gaits, we compared our method with prior methods for emotion and action recognition from gaits since these methods also solve the problem of gait classification (albeit with a different set of labels). We compare with approaches that use spatial-temporal graph convolution networks for emotion (STEP~\cite{bhattacharya2019step}) and action recognition (ST-GCN~\cite{yan2018spatial}). We also compare our method with an approach that uses a novel directed graph neural network (DGNN~\cite{shi2019skeleton}) for action recognition. We train these methods on our DeceptiveWalk dataset and obtain their performance on the testing set similar to our method. Our method outperforms these state-of-the-art models used for emotion and action recognition by a minimum of $4.7\%$ (Table~\ref{tab:accuracy}). We also conducted a subject independent study where the train and test datasets had different sets of participants. We observed accuracy of $85.06\%$ indicating that the accuracy of our algorithm does not depend on the participants.

Furthermore, we show the scatter of the features from both the natural and the deceptive classes in Figure~\ref{fig:scatter}. The original features are high dimensional ($f_{gait} \in \mathbb{R}^{29}, f_{gesture} \in \mathbb{R}^{7}$, and $f_d \in \mathbb{R}^{32}$). Hence we perform PCA to project and visualize them on a $3$ dimensional space. The gait and gesture features from the two classes are not separable in this space. However, the combined gait+gesture features, as well as the deep features from the two classes, are well-separated even in this lower-dimensional space, implying that the deep features ($f_d$) and gait+gesture features ($f_g$) can efficiently separate between the two classes.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/scatter.png}
    \caption{\textbf{Separation of Features}: We present the scatter plot of the features for each of the two-class labels. We project the features to a $3$ dimensional space using PCA for visualization. The gait and gesture features are not separable in this space. However, the combined gait+gestures features and deep features are well separated even in this low dimensional space. The boundary demarcated for the deceptive class features is only for visualization and does not represent the true class boundary.}
    \label{fig:scatter}
    % \vspace{-15pt}
\end{figure}

\subsection{Analysis of Gesture Cues}
% \begin{table}[t]
% \caption{\textbf{Gesture Features}: We present the percentage of videos in which the gestures were observed for both deceptive and natural walks. We observe that deceivers put their hands in their pockets and look around more than in the natural condition. However, the trend is unclear in other gestures. This could be explained in previous literature that suggests that deceivers try to alter or control what they think others are paying the most attention to~\protect\cite{EkmanNonverbalLeakage,DePauloCues,Navarro2003}. }
% \centering
% \begin{tabular}{|l|c|c|}
% \hline
% \multicolumn{1}{|c|}{Gesture} & Natural & Deceptive  \\ \hline
% One Hand In Pocket	& 7.87	& 16.98	  \\ \hline
% Two Hands In Pockets	& 5.51	& 22.01	  \\ \hline
% Looking Around	& 14.17	& 27.04	  \\ \hline
% Touching Face	& 6.30	& 6.92	  \\ \hline
% Touching Shirt/Jackets	& 7.87	& 1.89	  \\ \hline
% Touching Hair	& 3.94	& 5.66	  \\ \hline
% Hands Folded	& 3.94	& 3.14	  \\ \hline
% Looking At Phone/Watch	& 3.15	& 3.14	  \\ \hline
% \end{tabular}
% \vspace{-15pt}
% \label{tab:gestureDist}
% \end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{images/gestures.PNG}
    % \vspace{-10pt}
    \caption{\textbf{Gesture Features}: We present the percentage of videos in which the gestures were observed for both deceptive and natural walks. We observe that deceivers put their hands in their pockets and look around more than participants in the natural condition. However, the trend is unclear in other gestures. This could be explained in previous literature that suggests that deceivers try to alter or control what they think others are paying the most attention to~\protect\cite{EkmanNonverbalLeakage,DePauloCues,Navarro2003}.}
    \label{fig:gestureDist}
    \vspace{-15pt}
\end{figure}

We tabulate the distribution of various gestures in Figure~\ref{fig:gestureDist}. We can make interesting observations from this data. 
\begin{enumerate}
    \item Deceivers are more likely to put their hands in their pockets, look around and check if anyone is noticing them, touch their face, and look at their phone than the participants in the natural condition.
    \item Participants in the natural condition touched their shirt/jacket more than the deceivers.
    \item Deceivers touched their hair and folded their hands at about the same rate as those in the natural condition.
\end{enumerate}
Previous literature suggests that deceivers are sometimes very aware of the cues they are putting out and may, in turn, display the opposite of the expectation or display a controlled movement~\cite{EkmanNonverbalLeakage,DePauloCues,Navarro2003}. This would explain observations 2 and 3. Factors like how often a person lies or how aware they are of others' perceptions of them could contribute to whether they show fidgeting and nervous behavior or controlled and stable movements. These results are in accordance with the Hawthorne effect. However, more analysis is necessary to accurately predict the importance of each gesture in the prediction and expression of deception in real-world cases.

==> ECCV2020 Tanmay Deception/6_conclusion.tex <==
\section{Conclusion, Limitations, and Future Work}
We presented a novel method for distinguishing the deceptive walks of individuals from natural walks based on their walking style or pattern in videos. Based on our novel \textit{DeceptiveWalk} dataset, we train an LSTM-based classifier that classifies the \textit{deceptive features} and predicts whether an individual is performing a deceptive walk. We observe an accuracy of \accuracy~obtained using 10-fold cross-validation on $2224$ data points.

% We observe that in the deceptive condition, participants are more likely to put their hands in their pockets than those in the natural condition. Deceivers also look around and check if anyone is noticing them more than walkers in the natural condition. Our findings also support the findings of the previous literature that deceivers may control or alter their behavior cues~\cite{EkmanNonverbalLeakage,DePauloCues,Navarro2003}.

There are some limitations to our approach. Our approach is based on our dataset collected in a controlled university lab setting. Participants in the study were aware of the context of the experiment, and compared to real-world situations, the stakes were smaller in our experiment. This means that our results are preliminary and may not be directly applicable for detecting many kinds of deceptive walking behaviors in the real-world. We need considerable more investigation and research in terms of testing these ideas in all kind of situations. This would require collecting a large sample of unbiased video data in different real-world scenarios and analyzing them. While we present an algorithm that detects deception using walking, we do not claim that performing certain gestures and walking in a certain way conveys deception in all cases. Additionally, since our algorithm does not provide $100\%$ accuracy for classifying both deceptive and natural walking, there can be false positives and false negatives. Therefore, other data (manual intervention and/or using other modalities) should be considered before assigning a final deceptive or a natural label to the walking when using our method in real-world applications.

Since the accuracy of our algorithm depends on the accurate extraction of 3D poses, the algorithm may perform poorly in cases where pose estimation is inaccurate (e.g., occlusions, bad lighting). For this work, we manually annotate the gesture data. In the future, we would like to automatically annotate different gestures performed by the individual and automate the entire method. Additionally, our approach is limited to walking. In the future, we would like to extend our algorithm to more general cases that include a variety of activities and also consider factors such as gender, culture, age, disabilities, etc. The analysis of our data collection study reveals an interesting mapping between gestures and deception. However, this mapping may depend on other factors and we would like to explore the factors that govern the relationship between gestures and deception. Finally, we would like to combine our method with other verbal and non-verbal cues of deception (e.g., gazing, facial expressions, etc.) and compare the usefulness of body expressions to other cues in detecting deception. 
